Focused Dynamic Slicing for Large Applications using an Abstract Memory-Model

Dynamic slicing techniques compute program dependencies to find all statements that affect the value of a variable at a program point for a specific execution. Despite their many potential uses, applicability is limited by the fact that they typically cannot scale beyond small-sized applications. We believe that at the heart of this limitation is the use of memory references to identify data-dependencies. Particularly, working with memory references hinders distinct treatment of the code-to-be-sliced (e.g., classes the user has an interest in) from the rest of the code (including libraries and frameworks). The ability to perform a coarser-grained analysis for the code that is not under focus may provide performance gains and could become one avenue toward scalability. In this paper, we propose a novel approach that completely replaces memory reference registering and processing with a memory analysis model that works with program symbols (i.e., terms). In fact, this approach enables the alternative of not instrumenting -- thus, not generating any trace -- for code that is not part of the code-to-be-sliced. We report on an implementation of an abstract dynamic slicer for C\#, \textit{DynAbs}, and an evaluation that shows how large and relevant parts of Roslyn and Powershell -- two of the largest and modern C\# applications that can be found in GitHub -- can be sliced for their test cases assertions in at most a few minutes. We also show how reducing the code-to-be-sliced focus can bring important speedups with marginal relative precision loss.

==> resources/tablaRealApps.tex <==

% Subject
% Subcomponente - #Criterios 
% Layer/level one: #Stmt.- #Distinct Stmt. - Time - #Sliced - %Slice
% Full: Idem one 
%  + Cuánto más se tarda en %
%  + Cuántas líneas de menos tiene el slice original 
%  + Porcentaje de precisión ganado

\begin{table*}[h]
	\small
	\setlength\tabcolsep{3.3pt}
	\begin{tabular}
		{|p{25mm}|p{8mm}|
			p{5mm}|p{7mm}|p{7mm}|p{6mm}|p{2mm}|
			p{5mm}|p{9mm}|p{9mm}|p{9mm}|
			p{7mm}|p{7mm}|p{6mm}|p{2mm}|p{5mm}|p{9mm}|}
		\hline
		\multicolumn{2}{|l|}{ } & 
		\multicolumn{9}{|c|}{Code-to-be-sliced instrumentation only} & 
		\multicolumn{6}{|c|}{Extended  Instrumentation} \\
		\hline
		% General
		Test class files (.cs)& 
		Criteria &		
		% Layer 1
		Inst. (\%) & 
		ES & 
		Stmts. & 
		SS & 
		SS (\%) & 
		t (s) &
		ExtCalls &
		Speedup &
		Prec. loss (\%) &
		% Full core
		ES. & 
		Stmtss & 
		SS & 
		SS (\%) & 
		t (s) &
		ExtCalls \\
		\hline
		\multicolumn{17}{|l|}{Roslyn} \\
		\hline
		StatementParsingTests & \multicolumn{1}{|r|}{534} & \multicolumn{1}{|r|}{9.02} & \multicolumn{1}{|r|}{19270} & \multicolumn{1}{|r|}{1228} & \multicolumn{1}{|r|}{416} & \multicolumn{1}{|r|}{34} & \multicolumn{1}{|r|}{4} & \multicolumn{1}{|r|}{5396} & \multicolumn{1}{|r|}{x1} & \multicolumn{1}{|r|}{0.00} & \multicolumn{1}{|r|}{19338} & \multicolumn{1}{|r|}{1257} & \multicolumn{1}{|r|}{430} & \multicolumn{1}{|r|}{34} & \multicolumn{1}{|r|}{4} & \multicolumn{1}{|r|}{5416} \\
        TypeTests & \multicolumn{1}{|r|}{171} & \multicolumn{1}{|r|}{35.85} & \multicolumn{1}{|r|}{49211} & \multicolumn{1}{|r|}{3982} & \multicolumn{1}{|r|}{1586} & \multicolumn{1}{|r|}{40} & \multicolumn{1}{|r|}{24} & \multicolumn{1}{|r|}{10418} & \multicolumn{1}{|r|}{x2} & \multicolumn{1}{|r|}{-0.01} & \multicolumn{1}{|r|}{76391} & \multicolumn{1}{|r|}{6226} & \multicolumn{1}{|r|}{2634} & \multicolumn{1}{|r|}{42} & \multicolumn{1}{|r|}{53} & \multicolumn{1}{|r|}{17332} \\
        BindingTests & \multicolumn{1}{|r|}{67} & \multicolumn{1}{|r|}{14.41} & \multicolumn{1}{|r|}{3176} & \multicolumn{1}{|r|}{974} & \multicolumn{1}{|r|}{258} & \multicolumn{1}{|r|}{26} & \multicolumn{1}{|r|}{1} & \multicolumn{1}{|r|}{1077} & \multicolumn{1}{|r|}{x93} & \multicolumn{1}{|r|}{-0.13} & \multicolumn{1}{|r|}{105219} & \multicolumn{1}{|r|}{9040} & \multicolumn{1}{|r|}{2495} & \multicolumn{1}{|r|}{28} & \multicolumn{1}{|r|}{102} & \multicolumn{1}{|r|}{21756} \\
        FlowTests & \multicolumn{1}{|r|}{40} & \multicolumn{1}{|r|}{4.53} & \multicolumn{1}{|r|}{667} & \multicolumn{1}{|r|}{388} & \multicolumn{1}{|r|}{104} & \multicolumn{1}{|r|}{27} & \multicolumn{1}{|r|}{0} & \multicolumn{1}{|r|}{277} & \multicolumn{1}{|r|}{x218} & \multicolumn{1}{|r|}{0.00} & \multicolumn{1}{|r|}{106715} & \multicolumn{1}{|r|}{8851} & \multicolumn{1}{|r|}{2736} & \multicolumn{1}{|r|}{31} & \multicolumn{1}{|r|}{83} & \multicolumn{1}{|r|}{20927} \\
        CompilationEmitTests & \multicolumn{1}{|r|}{99} & \multicolumn{1}{|r|}{6.32} & \multicolumn{1}{|r|}{3582} & \multicolumn{1}{|r|}{887} & \multicolumn{1}{|r|}{280} & \multicolumn{1}{|r|}{32} & \multicolumn{1}{|r|}{2} & \multicolumn{1}{|r|}{2381} & \multicolumn{1}{|r|}{x81} & \multicolumn{1}{|r|}{0.00} & \multicolumn{1}{|r|}{105464} & \multicolumn{1}{|r|}{7045} & \multicolumn{1}{|r|}{1977} & \multicolumn{1}{|r|}{28} & \multicolumn{1}{|r|}{128} & \multicolumn{1}{|r|}{28378} \\
        %PDBTests.cs & \multicolumn{1}{|r|}{414} & \multicolumn{1}{|r|}{35.85} & \multicolumn{1}{|r|}{103127} & \multicolumn{1}{|r|}{6039} & \multicolumn{1}{|r|}{2009} & \multicolumn{1}{|r|}{33} & \multicolumn{1}{|r|}{88} & \multicolumn{1}{|r|}{22484} & \multicolumn{1}{|r|}{x2} & \multicolumn{1}{|r|}{0.00} & \multicolumn{1}{|r|}{137648} & \multicolumn{1}{|r|}{9011} & \multicolumn{1}{|r|}{2992} & \multicolumn{1}{|r|}{33} & \multicolumn{1}{|r|}{176} & \multicolumn{1}{|r|}{30749} \\

		\hline
		\multicolumn{17}{|l|}{Powershell} \\
		\hline		
		FileSystemProvider & \multicolumn{1}{|r|}{13} & \multicolumn{1}{|r|}{4.89} & \multicolumn{1}{|r|}{14410} & \multicolumn{1}{|r|}{633} & \multicolumn{1}{|r|}{13} & \multicolumn{1}{|r|}{2} & \multicolumn{1}{|r|}{2} & \multicolumn{1}{|r|}{6388} & \multicolumn{1}{|r|}{x91} & \multicolumn{1}{|r|}{0.00} & \multicolumn{1}{|r|}{151088} & \multicolumn{1}{|r|}{4972} & \multicolumn{1}{|r|}{1630} & \multicolumn{1}{|r|}{33} & \multicolumn{1}{|r|}{214} & \multicolumn{1}{|r|}{38626} \\
        MshSnapinInfo & \multicolumn{1}{|r|}{1} & \multicolumn{1}{|r|}{0.28} & \multicolumn{1}{|r|}{96} & \multicolumn{1}{|r|}{104} & \multicolumn{1}{|r|}{6} & \multicolumn{1}{|r|}{6} & \multicolumn{1}{|r|}{0} & \multicolumn{1}{|r|}{39} & \multicolumn{1}{|r|}{x2} & \multicolumn{1}{|r|}{0.00} & \multicolumn{1}{|r|}{557} & \multicolumn{1}{|r|}{493} & \multicolumn{1}{|r|}{20} & \multicolumn{1}{|r|}{4} & \multicolumn{1}{|r|}{0} & \multicolumn{1}{|r|}{201} \\
        NamedPipe & \multicolumn{1}{|r|}{4} & \multicolumn{1}{|r|}{14.88} & \multicolumn{1}{|r|}{209} & \multicolumn{1}{|r|}{156} & \multicolumn{1}{|r|}{5} & \multicolumn{1}{|r|}{3} & \multicolumn{1}{|r|}{0} & \multicolumn{1}{|r|}{71} & \multicolumn{1}{|r|}{x1} & \multicolumn{1}{|r|}{0.00} & \multicolumn{1}{|r|}{299} & \multicolumn{1}{|r|}{203} & \multicolumn{1}{|r|}{6} & \multicolumn{1}{|r|}{3} & \multicolumn{1}{|r|}{0} & \multicolumn{1}{|r|}{91} \\
        CorePsPlatform & \multicolumn{1}{|r|}{1} & \multicolumn{1}{|r|}{3.30} & \multicolumn{1}{|r|}{9} & \multicolumn{1}{|r|}{13} & \multicolumn{1}{|r|}{2} & \multicolumn{1}{|r|}{15} & \multicolumn{1}{|r|}{0} & \multicolumn{1}{|r|}{15} & \multicolumn{1}{|r|}{x1} & \multicolumn{1}{|r|}{0.00} & \multicolumn{1}{|r|}{9} & \multicolumn{1}{|r|}{13} & \multicolumn{1}{|r|}{2} & \multicolumn{1}{|r|}{15} & \multicolumn{1}{|r|}{0} & \multicolumn{1}{|r|}{15} \\
        PowerShellAPI & \multicolumn{1}{|r|}{3} & \multicolumn{1}{|r|}{4.16} & \multicolumn{1}{|r|}{1728} & \multicolumn{1}{|r|}{1066} & \multicolumn{1}{|r|}{491} & \multicolumn{1}{|r|}{46} & \multicolumn{1}{|r|}{1} & \multicolumn{1}{|r|}{200} & \multicolumn{1}{|r|}{x981} & \multicolumn{1}{|r|}{0.00} & \multicolumn{1}{|r|}{225696} & \multicolumn{1}{|r|}{9740} & \multicolumn{1}{|r|}{5028} & \multicolumn{1}{|r|}{52} & \multicolumn{1}{|r|}{826} & \multicolumn{1}{|r|}{55633} \\
        PSConfiguration & \multicolumn{1}{|r|}{286} & \multicolumn{1}{|r|}{0.10} & \multicolumn{1}{|r|}{312} & \multicolumn{1}{|r|}{171} & \multicolumn{1}{|r|}{44} & \multicolumn{1}{|r|}{26} & \multicolumn{1}{|r|}{0} & \multicolumn{1}{|r|}{97} & \multicolumn{1}{|r|}{x2} & \multicolumn{1}{|r|}{-1.63} & \multicolumn{1}{|r|}{642} & \multicolumn{1}{|r|}{254} & \multicolumn{1}{|r|}{54} & \multicolumn{1}{|r|}{21} & \multicolumn{1}{|r|}{0} & \multicolumn{1}{|r|}{203} \\
        Binders & \multicolumn{1}{|r|}{1} & \multicolumn{1}{|r|}{4.00} & \multicolumn{1}{|r|}{12} & \multicolumn{1}{|r|}{18} & \multicolumn{1}{|r|}{4} & \multicolumn{1}{|r|}{22} & \multicolumn{1}{|r|}{0} & \multicolumn{1}{|r|}{14} & \multicolumn{1}{|r|}{x1} & \multicolumn{1}{|r|}{0.00} & \multicolumn{1}{|r|}{12} & \multicolumn{1}{|r|}{18} & \multicolumn{1}{|r|}{4} & \multicolumn{1}{|r|}{22} & \multicolumn{1}{|r|}{0} & \multicolumn{1}{|r|}{14} \\
        PSObject & \multicolumn{1}{|r|}{15} & \multicolumn{1}{|r|}{1.19} & \multicolumn{1}{|r|}{496} & \multicolumn{1}{|r|}{299} & \multicolumn{1}{|r|}{78} & \multicolumn{1}{|r|}{26} & \multicolumn{1}{|r|}{0} & \multicolumn{1}{|r|}{91} & \multicolumn{1}{|r|}{x45} & \multicolumn{1}{|r|}{0.00} & \multicolumn{1}{|r|}{8456} & \multicolumn{1}{|r|}{1206} & \multicolumn{1}{|r|}{416} & \multicolumn{1}{|r|}{35} & \multicolumn{1}{|r|}{4} & \multicolumn{1}{|r|}{2596} \\
        ExtensionMethods & \multicolumn{1}{|r|}{1} & \multicolumn{1}{|r|}{3.72} & \multicolumn{1}{|r|}{98} & \multicolumn{1}{|r|}{76} & \multicolumn{1}{|r|}{21} & \multicolumn{1}{|r|}{28} & \multicolumn{1}{|r|}{0} & \multicolumn{1}{|r|}{23} & \multicolumn{1}{|r|}{x6} & \multicolumn{1}{|r|}{-23.68} & \multicolumn{1}{|r|}{3290} & \multicolumn{1}{|r|}{214} & \multicolumn{1}{|r|}{6} & \multicolumn{1}{|r|}{3} & \multicolumn{1}{|r|}{1} & \multicolumn{1}{|r|}{1236} \\
        PSVersionInfo & \multicolumn{1}{|r|}{1} & \multicolumn{1}{|r|}{0.17} & \multicolumn{1}{|r|}{202} & \multicolumn{1}{|r|}{149} & \multicolumn{1}{|r|}{11} & \multicolumn{1}{|r|}{7} & \multicolumn{1}{|r|}{0} & \multicolumn{1}{|r|}{60} & \multicolumn{1}{|r|}{x1} & \multicolumn{1}{|r|}{0.00} & \multicolumn{1}{|r|}{202} & \multicolumn{1}{|r|}{149} & \multicolumn{1}{|r|}{11} & \multicolumn{1}{|r|}{7} & \multicolumn{1}{|r|}{0} & \multicolumn{1}{|r|}{60} \\
        Runspace & \multicolumn{1}{|r|}{9} & \multicolumn{1}{|r|}{8.37} & \multicolumn{1}{|r|}{2536} & \multicolumn{1}{|r|}{1130} & \multicolumn{1}{|r|}{548} & \multicolumn{1}{|r|}{48} & \multicolumn{1}{|r|}{1} & \multicolumn{1}{|r|}{615} & \multicolumn{1}{|r|}{x38} & \multicolumn{1}{|r|}{0.00} & \multicolumn{1}{|r|}{105198} & \multicolumn{1}{|r|}{6388} & \multicolumn{1}{|r|}{2715} & \multicolumn{1}{|r|}{43} & \multicolumn{1}{|r|}{34} & \multicolumn{1}{|r|}{26848} \\
        SecuritySupport & \multicolumn{1}{|r|}{1} & \multicolumn{1}{|r|}{1.33} & \multicolumn{1}{|r|}{41} & \multicolumn{1}{|r|}{48} & \multicolumn{1}{|r|}{20} & \multicolumn{1}{|r|}{42} & \multicolumn{1}{|r|}{0} & \multicolumn{1}{|r|}{15} & \multicolumn{1}{|r|}{x2} & \multicolumn{1}{|r|}{0.00} & \multicolumn{1}{|r|}{104} & \multicolumn{1}{|r|}{115} & \multicolumn{1}{|r|}{23} & \multicolumn{1}{|r|}{20} & \multicolumn{1}{|r|}{0} & \multicolumn{1}{|r|}{51} \\
        SessionState & \multicolumn{1}{|r|}{1} & \multicolumn{1}{|r|}{67.98} & \multicolumn{1}{|r|}{159105} & \multicolumn{1}{|r|}{6217} & \multicolumn{1}{|r|}{4} & \multicolumn{1}{|r|}{0} & \multicolumn{1}{|r|}{165} & \multicolumn{1}{|r|}{40947} & \multicolumn{1}{|r|}{x1} & \multicolumn{1}{|r|}{0.00} & \multicolumn{1}{|r|}{179189} & \multicolumn{1}{|r|}{7527} & \multicolumn{1}{|r|}{4} & \multicolumn{1}{|r|}{0} & \multicolumn{1}{|r|}{220} & \multicolumn{1}{|r|}{49350} \\
        Utils & \multicolumn{1}{|r|}{45} & \multicolumn{1}{|r|}{0.40} & \multicolumn{1}{|r|}{20} & \multicolumn{1}{|r|}{9} & \multicolumn{1}{|r|}{5} & \multicolumn{1}{|r|}{54} & \multicolumn{1}{|r|}{0} & \multicolumn{1}{|r|}{17} & \multicolumn{1}{|r|}{x16} & \multicolumn{1}{|r|}{0.00} & \multicolumn{1}{|r|}{1619} & \multicolumn{1}{|r|}{223} & \multicolumn{1}{|r|}{8} & \multicolumn{1}{|r|}{4} & \multicolumn{1}{|r|}{0} & \multicolumn{1}{|r|}{609} \\
        WildcardPattern & \multicolumn{1}{|r|}{13} & \multicolumn{1}{|r|}{0.22} & \multicolumn{1}{|r|}{6} & \multicolumn{1}{|r|}{10} & \multicolumn{1}{|r|}{2} & \multicolumn{1}{|r|}{17} & \multicolumn{1}{|r|}{0} & \multicolumn{1}{|r|}{1} & \multicolumn{1}{|r|}{x1} & \multicolumn{1}{|r|}{0.00} & \multicolumn{1}{|r|}{12} & \multicolumn{1}{|r|}{18} & \multicolumn{1}{|r|}{3} & \multicolumn{1}{|r|}{17} & \multicolumn{1}{|r|}{0} & \multicolumn{1}{|r|}{2} \\
		\hline
	\end{tabular}
	\caption{Execution results. $Criteria$ is the number of slicing criteria used, $Inst. (\%)$ is the percentage of instrumented compared to that instrumented in the "Extended Instrumentation", $ES$ is the average execution size in \# of statements, 	$Stmts.$ is the average number of unique statements that can be sliced, $SS$ is the average number of statements in the slice and  $SS (\%)$ is $SS\Stmts.$, $t$ is the average slice computation time in seconds, $ExtCalls$ is the average number of calls that were \textit{havoc}-ed, and $Speedup$ and $Prec. loss$ are the slicing speedup time and precision loss percentage of the less instrumented code compared to the slicing of the code with extended instrumentationc\su{La columna inst debería ser la columna justo antes de speed up}}
	\label{tab:tablePSRoslyn}
\end{table*}
